Inferring Inductive Invariants from Phase Structures

Infinite-state systems such as distributed protocols are challenging to verify using interactive theorem provers or automatic verification tools. Of these techniques, deductive verification is highly expressive but requires the user to annotate the system with inductive invariants. To relieve the user from this labor-intensive and challenging task, invariant inference aims to find inductive invariants automatically. Unfortunately, when applied to infinite-state systems such as distributed protocols, existing inference techniques often diverge, which limits their applicability. This paper proposes user-guided invariant inference based on phase invariants, which capture the different logical phases of the protocol. Users conveys their intuition by specifying a phase structure, an automaton with edges labeled by program transitions; the tool automatically infers assertions that hold in the automaton's states, resulting in a full safety proof.The additional structure from phases guides the inference procedure towards finding an invariant. Our results show that user guidance by phase structures facilitates successful inference beyond the state of the art. We find that phase structures are pleasantly well matched to the intuitive reasoning routinely used by domain experts to understand why distributed protocols are correct, so that providing a phase structure reuses this existing intuition.

==> figs/sharded-kv-automaton-w-char-short.tex <==
\begin{figure*}[t]
\begin{subfigure}{\textwidth}
  \centering
  %\includegraphics[width=3in]{figs/lockserv-automaton-labeled-states}
  \begin{tikzpicture}[
    state/.style={
      draw,
      circle,
      font=\footnotesize\ttfamily,
      minimum size=9mm,
      inner sep=0pt
    },
    action/.style={
      font=\ttfamily\scriptsize %\color{red}
    }
  ]
    \node[state] (O) at (180:1.5cm) {{\small O[$k$]}};
    \node[state] (T) at (0:1.5cm) {{\small T[$k$]}};

    \draw[->] (O) edge[bend left] node[action,above] {\footnotesize reshard(*,*,$k$,*)} (T);
    %\draw[->] (G) edge[bend left]  node[action,below right] {recv\_grant(*,$\lockelem$)} (HL);
    %\draw[->] (HL) edge[bend left] node[action,below left] {send\_unlock(*,$\lockelem$)} (U);
    \draw[->] (T) edge[bend left] node[action,below] {\footnotesize recv\_transfer\_msg(*,*,$k$,*,*)} (O);

    \draw[->] (O) edge[loop left] node[action,left,align=center] 
      {drop\_transfer\_msg(*,*,$k$,*,*) \\
       retransmit(*,*,$k$,*,*) \\
       send\_ack(*,*,$k$,*,*) \\
       drop\_ack\_msg(*,*,$k$,*) \\
       recv\_ack\_msg(*,*,$k$,*) \\
       put(*,$k$,*)} (O);
    \draw[->] (T) edge[loop right] node[action,right,align=center] 
      {drop\_transfer\_msg(*,*,$k$,*,*) \\
       retransmit(*,*,$k$,*,*) \\
       send\_ack(*,*,$k$,*,*) \\
       drop\_ack\_msg(*,*,$k$,*) \\
       recv\_ack\_msg(*,*,$k$,*) \\
       put(*,$k$,*)} (T);
  \end{tikzpicture}
  %\caption{Phase automaton for the lock service. Clockwise from top, the
%    phases for the lock $\lockelem$ are: Server Holds Lock, \texttt{Grant} message destined for some client, lock held by some client, and \texttt{Unlock} message sent from some client and pending to be received by the server.  The transitions are labeled by actions of the system. The wildcard * means that the action is executed by some arbitrary node (in the transition relation this is translated to an existential quantifier). Each phase has
%    a self loop for \texttt{send\_lock}, which can happen at any time. Actions related to locks other than $\lockelem$ are considered as self-loops, and omitted here for brevity \TODO{clear?}. There
%    are four non-self-loop edges, forming the core of the automaton and
%    capturing the lifecycle of the lock service. Not all actions are allowed
%    in every phase: only those actions with outgoing edges are allowed. Our
%    inference algorithm exploits missing edges as additional safety properties
%    to guide the search.
%  }
  %\label{fig:lockserv-automaton}
\end{subfigure}
\\
\begin{subfigure}{\textwidth}
  \centering
  \begin{lstlisting}[numbers=left, numberstyle=\tiny, numbersep=5pt, name=lockserv, morekeywords={phase}]
phase O[$k$]:
  invariant $\forall n_1,n_2.$ owner($n_1$,$k$)$\land$owner($n_2$,$k$)$\rightarrow n_1=n_2$
  invariant $\forall n,v.$ table($n$,$k$,$v$)$\rightarrow$owner($n$,$k$)
  invariant $\forall \vsrc,\vdst,v,s.$ $\neg$(transfer_msg($\vsrc$,$\vdst$,$k$,$v$,$s$)$\land$$\neg$seqnum_recvd($\vdst$,$\vsrc$,$s$))$\label{kv-char:disallow-recv-transfer}$
  invariant $\forall n_1,n_2,v_1,v_2.$ table($n_1$,$k$,$v_1$)$\land$table($n_2$,$k$,$v_2$)$\rightarrow n_1 = n_2 \land v_1 = v_2$
  invariant $\forall \vsrc,\vdst,v,s.$ $\neg$(unacked($\vsrc$,$\vdst$,$k$,$v$,$s$)$\land$$\neg$seqnum_recvd($\vdst$,$\vsrc$,$s$))

phase T[$k$]:
  invariant $\forall n.$ $\neg$owner($n$,$k$)
  invariant $\forall n,v.$ table($n$,$k$,$v$)$\rightarrow$owner($n$,$k$)
  invariant $\label{kv-char:unique-transfer-unreceived}$$\forall \vsrc_1,\vsrc_2,\vdst_1,\vdst_2,v_1,v_2,s_1,s_2.$ transfer_msg($\vsrc_1$,$\vdst_1$,$k$,$v_1$,$s_1$)$\land$$\neg$seqnum_recvd($\vdst_1$,$\vsrc_1$,$s_1$)
    $\land$transfer_msg($\vsrc_2$,$\vdst_2$,$k$,$v_2$,$s_2$)$\land$$\neg$seqnum_recvd($\vdst_2$,$\vsrc_2$,$s_2$)$\rightarrow (\vsrc_1, \vdst_1, v_1, s_1)=(\vsrc_2, \vdst_2, v_2, s_2)$
  invariant $\forall \vsrc_1,\vsrc_2,\vdst_1,\vdst_2,v_1,v_2,s_1,s_2.$transfer_msg($\vsrc_1$,$\vdst_1$,$k$,$v_1$,$s_1$)$\land$$\neg$seqnum_recvd($\vdst_1$,$\vdst_1$,$s_1$)
    $\land$unacked($\vsrc_2$,$\vdst_2$,$k$,$v_2$,$s_2$)$\land$$\neg$seqnum_recvd($\vdst_2$,$\vsrc_2$,$s_2$)$\rightarrow (\vsrc_1, \vdst_1, v_1, s_1) = (\vsrc_2, \vdst_2, v_2, s_2)$
  invariant $\forall \vsrc_1,\vsrc_2,\vdst_1,\vdst_2,v_1,v_2,s_1,s_2.$ unacked($\vsrc_1$,$\vdst_1$,$k$,$v_1$,$s_1$)$\land$$\neg$seqnum_recvd($\vdst_1$,$\vsrc_1$,$s_1$)
    $\land$unacked($\vsrc_2$,$\vdst_2$,$k$,$v_2$,$s_2$)$\land$$\neg$seqnum_recvd($\vdst_2$,$\vsrc_2$,$s_2$)$\rightarrow (\vsrc_1, \vdst_1, v_1, s_1) = (\vsrc_2, \vdst_2, v_2, s_2)$
\end{lstlisting}
  %\caption{Logical characterizations of the automaton states to prove it inductive.
%    \TODO{Emphasize how the characterizations are (1) natural and (2) intuitive. But seriously,
%    each one says that exactly one out of four pieces of state is ``active'' while the others are ``passive''.}}
%  \label{fig:lockserv-invariants}
%  \label{fig:lockservice-phase}
\end{subfigure}
\caption{\footnotesize Phase structure for key-value store (top) and phase characterizations (bottom). The user provides the phase structure, and inference automatically produces the phase characterizations, forming a safe inductive phase automaton.
}
\label{fig:kv-automaton}
\label{fig:kv-invariants}
\label{fig:kv-phase}
\end{figure*} 

==> figs/sharded-kv-automaton-w-char.tex <==
\begin{figure*}[t]
\begin{subfigure}{\textwidth}
  \centering
  %\includegraphics[width=3in]{figs/lockserv-automaton-labeled-states}
  \begin{tikzpicture}[
    state/.style={
      draw,
      circle,
      font=\footnotesize\ttfamily,
      minimum size=9mm,
      inner sep=0pt
    },
    action/.style={
      font=\ttfamily\scriptsize %\color{red}
    }
  ]
    \node[state] (O) at (180:1.5cm) {{\small O[$k$]}};
    \node[state] (T) at (0:1.5cm) {{\small T[$k$]}};

    \draw[->] (O) edge[bend left] node[action,above] {\footnotesize reshard(*,*,$k$,*)} (T);
    %\draw[->] (G) edge[bend left]  node[action,below right] {recv\_grant(*,$\lockelem$)} (HL);
    %\draw[->] (HL) edge[bend left] node[action,below left] {send\_unlock(*,$\lockelem$)} (U);
    \draw[->] (T) edge[bend left] node[action,below] {\footnotesize recv\_transfer\_msg(*,*,$k$,*,*)} (O);

    \draw[->] (O) edge[loop left] node[action,left,align=center] 
      {drop\_transfer\_msg(*,*,$k$,*,*) \\
       retransmit(*,*,$k$,*,*) \\
       send\_ack(*,*,$k$,*,*) \\
       drop\_ack\_msg(*,*,$k$,*) \\
       recv\_ack\_msg(*,*,$k$,*) \\
       put(*,$k$,*)} (O);
    \draw[->] (T) edge[loop right] node[action,right,align=center] 
      {drop\_transfer\_msg(*,*,$k$,*,*) \\
       retransmit(*,*,$k$,*,*) \\
       send\_ack(*,*,$k$,*,*) \\
       drop\_ack\_msg(*,*,$k$,*) \\
       recv\_ack\_msg(*,*,$k$,*) \\
       put(*,$k$,*)} (T);
  \end{tikzpicture}
  %\caption{Phase automaton for the lock service. Clockwise from top, the
%    phases for the lock $\lockelem$ are: Server Holds Lock, \texttt{Grant} message destined for some client, lock held by some client, and \texttt{Unlock} message sent from some client and pending to be received by the server.  The transitions are labeled by actions of the system. The wildcard * means that the action is executed by some arbitrary node (in the transition relation this is translated to an existential quantifier). Each phase has
%    a self loop for \texttt{send\_lock}, which can happen at any time. Actions related to locks other than $\lockelem$ are considered as self-loops, and omitted here for brevity \TODO{clear?}. There
%    are four non-self-loop edges, forming the core of the automaton and
%    capturing the lifecycle of the lock service. Not all actions are allowed
%    in every phase: only those actions with outgoing edges are allowed. Our
%    inference algorithm exploits missing edges as additional safety properties
%    to guide the search.
%  }
  %\label{fig:lockserv-automaton}
\end{subfigure}
\\
\begin{subfigure}{\textwidth}
  \centering
  \begin{lstlisting}[numbers=left, numberstyle=\tiny, numbersep=5pt, name=lockserv, morekeywords={phase}]
phase O[$k$]:
  invariant $\forall n_1,n_2.$ owner($n_1$,$k$)$\land$owner($n_2$,$k$)$\rightarrow n_1=n_2$
  invariant $\forall n,v.$ table($n$,$k$,$v$)$\rightarrow$owner($n$,$k$)
  invariant $\forall \vsrc,\vdst,v,s.$ $\neg$(transfer_msg($\vsrc$,$\vdst$,$k$,$v$,$s$)$\land$$\neg$seqnum_recvd($\vdst$,$\vsrc$,$s$))$\label{kv-char:disallow-recv-transfer}$
  invariant $\forall n_1,n_2,v_1,v_2.$ table($n_1$,$k$,$v_1$)$\land$table($n_2$,$k$,$v_2$)$\rightarrow n_1 = n_2 \land v_1 = v_2$
  invariant $\forall \vsrc,\vdst,v,s.$ $\neg$(unacked($\vsrc$,$\vdst$,$k$,$v$,$s$)$\land$$\neg$seqnum_recvd($\vdst$,$\vsrc$,$s$))

phase T[$k$]:
  invariant $\forall n.$ $\neg$owner($n$,$k$)
  invariant $\forall n,v.$ table($n$,$k$,$v$)$\rightarrow$owner($n$,$k$)
  invariant $\label{kv-char:unique-transfer-unreceived}$$\forall \vsrc_1,\vsrc_2,\vdst_1,\vdst_2,v_1,v_2,s_1,s_2.$ transfer_msg($\vsrc_1$,$\vdst_1$,$k$,$v_1$,$s_1$)$\land$$\neg$seqnum_recvd($\vdst_1$,$\vsrc_1$,$s_1$)
    $\land$transfer_msg($\vsrc_2$,$\vdst_2$,$k$,$v_2$,$s_2$)$\land$$\neg$seqnum_recvd($\vdst_2$,$\vsrc_2$,$s_2$)$\rightarrow \vsrc_1 = \vsrc_2 \land \vdst_1 = \vdst_2 \land v_1=v_2 \land s_1=s_2$
  invariant $\forall \vsrc_1,\vsrc_2,\vdst_1,\vdst_2,v_1,v_2,s_1,s_2.$transfer_msg($\vsrc_1$,$\vdst_1$,$k$,$v_1$,$s_1$)$\land$$\neg$seqnum_recvd($\vdst_1$,$\vdst_1$,$s_1$)
    $\land$unacked($\vsrc_2$,$\vdst_2$,$k$,$v_2$,$s_2$)$\land$$\neg$seqnum_recvd($\vdst_2$,$\vsrc_2$,$s_2$)$\rightarrow \vsrc_1 = \vsrc_2 \land \vdst_1 \land \vdst_2 \land v_1 = v_2 \land s_1 = s_2$
  invariant $\forall \vsrc_1,\vsrc_2,\vdst_1,\vdst_2,v_1,v_2,s_1,s_2.$ unacked($\vsrc_1$,$\vdst_1$,$k$,$v_1$,$s_1$)$\land$$\neg$seqnum_recvd($\vdst_1$,$\vsrc_1$,$s_1$)
    $\land$unacked($\vsrc_2$,$\vdst_2$,$k$,$v_2$,$s_2$)$\land$$\neg$seqnum_recvd($\vdst_2$,$\vsrc_2$,$s_2$)$\rightarrow \vsrc_1 = \vsrc_2 \land \vdst_1 = \vdst_2 \land v_1 = v_2 \land s_1 = s_2$
\end{lstlisting}
  %\caption{Logical characterizations of the automaton states to prove it inductive.
%    \TODO{Emphasize how the characterizations are (1) natural and (2) intuitive. But seriously,
%    each one says that exactly one out of four pieces of state is ``active'' while the others are ``passive''.}}
%  \label{fig:lockserv-invariants}
%  \label{fig:lockservice-phase}
\end{subfigure}
\caption{\footnotesize Phase structure for key-value store (top) and phase characterizations (bottom). The user provides the phase structure, and inference automatically produces the phase characterizations, forming a safe inductive phase automaton.
}
\label{fig:kv-automaton}
\label{fig:kv-invariants}
\label{fig:kv-phase}
\end{figure*} 

==> figs/sharded-kv-code-short.tex <==

\begin{figure*}[t]
  \centering
\begin{minipage}{1.1\textwidth}
%  \begin{subfigure}[t]{0.35\textwidth}
  \begin{minipage}{0.53\textwidth}
  \begin{lstlisting}[numbers=left, numberstyle=\tiny, numbersep=5pt, name=lockserv, escapeinside={(*}{*)}]
type key(*\label{kv-code:types-start}*)
type value
type node
type sequnum(*\label{kv-code:types-end}*)

relation owner: node, key(*\label{kv-code:state-start}*)
relation table: node, key, value
relation transfer_msg: node, node, 
                       key, value, seqnum
relation ack_msg: node, node, seqnum
relation seqnum_sent: node, seqnum
relation unacked: node, node, 
                  key, value, seqnum
relation seqnum_recvd: node, node, seqnum(*\label{kv-code:state-end}*)

init $\forall n_1,n_2,k.$(*\label{kv-code:init-start}*) owner($n_1$,$k$)$\land$owner($n_2$,$k$)
                  $\rightarrow n_1=n_2$(*\label{kv-code:init-start}*)
init // all other relations are empty(*\label{kv-code:init-end}*)

action reshard(n_old:node, n_new:node,(*\label{kv-code:action-start}*)(*\label{kv-code:reshard-start}*)
               k:key, value:sequnum)
  require table(n_old, k, v)
        $\land$$\neg$seqnum_sent(n_old, s)
  seqnum_sent(n_old, s) := true
  table(n_old, k, v) := false
  owner(n_old, k) := false(*\label{kv-code:cede-own}*)
  transfer_msg(n_old, n_new, k, v, s) := true(*\label{kv-code:inserting-tuple}*)
  unacked(n_old, n_new, k, v, s) := true(*\label{kv-code:reshard-end}*)

action drop_transfer_msg(src:node, dst:node,(*\label{kv-code:transfer-drop-start}*)
                    k:key, v:value, s:seqnum)
    require transfer_msg(src, dst, k, v, s)(*\label{kv-code:requiring-tuple}*)
    transfer_msg(src, dst, k, v, s) := false(*\label{kv-code:removing-tuple}*)(*\label{kv-code:transfer-drop-end}*)

action retransmit(src:node, dst:node,(*\label{kv-code:transfer-retransmit-start}*)
                  k:key, v:value, s:seqnum)
    require unacked(src, dst, k, v, s)
    transfer_msg(src, dst, k, v, s) := true(*\label{kv-code:transfer-retransmit-end}*)
  \end{lstlisting}
  %\end{subfigure}%
  \end{minipage}
\hspace{0.0\textwidth}%
%\begin{subfigure}[t]{0.28\textwidth}
\begin{minipage}{0.4\textwidth}
  \begin{lstlisting}[numbers=left, numberstyle=\tiny, numbersep=5pt, name=lockserv, escapeinside={(*}{*)}]
action recv_transfer_msg(src:node, n:node,(*\label{kv-code:receive-transfer-start}*)
              k:key, v:value, s:seqnum)
    require transfer_msg(src, n, k, v, s)
          $\land$$\neg$seqnum_recvd(n, src, s)(*\label{kv-code:ignore-dup}*)
    seqnum_recvd(n, src, s) := true
    table(n, k, v) := true
    owner(n, k) := true(*\label{kv-code:receive-transfer-end}*)

action send_ack(src:node, n:node,(*\label{kv-code:ack-start}*)
              k:key, v:value, s:seqnum)
    require transfer_msg(src, n, k, v, s)
          $\land$seqnum_recvd(n, src, s)
    ack_msg(src, n, s) := true(*\label{kv-code:ack-end}*)

action drop_ack_msg(src:node, dst:node,(*\label{kv-code:ack-drop-start}*)
              k:key, s:seqnum)
    require ack_msg(src, dst, s)
    ack_msg(src, dst, s) := false(*\label{kv-code:ack-drop-end}*)

action recv_ack_msg(src:node, dst:node, 
              k:key, s:seqnum)
    require ack_msg(src, dst, s)
    unacked(src, dst, *, *, s) := false(*\label{kv-code:qf-update:recv_ack_msg}*)

action put(n:node, k:key, v:value)
    require owner(n, k)
    table(n, k, *) := false(*\label{kv-code:qf-update:put}*)
    table(n, k, v) := true(*\label{kv-code:action-end}*)

safety $\forall k, n_1, n_2, v_1, v_2.$(*\label{kv-code:safety-start}*)
  table($n_1$,$k$,$v_1$) $\land$
  table($n_2$,$k$,$v_2$) $\to$
  $n_1 = n_2 \land v_1 = v_2$(*\label{kv-code:safety-end}*)
  \end{lstlisting}
%  \end{subfigure}
\end{minipage}
\captionof{figure}{\footnotesize Sharded key-value store with retransmissions (KV-R) in a first-order relational modeling.}
  \label{fig:kv-ivy}
  \end{minipage}
%  \begin{subfigure}[t]{0.3\textwidth}  %\caption{Lock service modeled in Ivy (left) and logical phase characterizations to prove it inductive (right) .}
\end{figure*} 

%\caption{Phase automaton for the lock service (left) and logical phase characterizations to prove it inductive (right).
%    Clockwise from top, the
%    phases for the lock $\lockelem$ are: Server Holds Lock, Grant message destined for some client, lock held by some client, and Unlock message sent from some client and pending to be received by the server.  The transitions are labeled by actions of the system. The wildcard \texttt{*} means that the action is executed by some arbitrary node.
%    %(in the transition relation this is translated to an existential quantifier).
%    Each phase has
%    a self loop for \texttt{send\_lock}, which can happen at any time. Actions related to locks other than $\lockelem$ are considered as self-loops, and omitted here for brevity. There
%    are four non-self-loop edges, forming the core of the automaton and
%    capturing the lifecycle of the lock service. Not all actions are allowed
%    in every phase: only those actions with outgoing edges are allowed. Our
%    inference algorithm exploits missing edges as additional safety properties
%    to guide the search.
%  }

==> figs/sharded-kv-code.tex <==

\begin{figure*}[t]
  \centering
\begin{minipage}{1.1\textwidth}
%  \begin{subfigure}[t]{0.35\textwidth}
  \begin{minipage}{0.53\textwidth}
  \begin{lstlisting}[numbers=left, numberstyle=\tiny, numbersep=5pt, name=lockserv, escapeinside={(*}{*)}]
type key(*\label{kv-code:types-start}*)
type value
type node
type sequnum(*\label{kv-code:types-end}*)

relation owner: node, key(*\label{kv-code:state-start}*)
relation table: node, key, value
relation transfer_msg: node, node, 
                       key, value, seqnum
relation ack_msg: node, node, seqnum
relation seqnum_sent: node, seqnum
relation unacked: node, node, 
                  key, value, seqnum
relation seqnum_recvd: node, node, seqnum(*\label{kv-code:state-end}*)

init $\forall n_1,n_2,k.$(*\label{kv-code:init-start}*) owner($n_1$,$k$)$\land$owner($n_2$,$k$)
                  $\rightarrow n_1=n_2$(*\label{kv-code:init-start}*)
init // all other relations are empty(*\label{kv-code:init-end}*)

action reshard(n_old:node, n_new:node,(*\label{kv-code:action-start}*)(*\label{kv-code:reshard-start}*)
               k:key, value:sequnum)
  require table(n_old, k, v)
        $\land$$\neg$seqnum_sent(n_old, s)
  seqnum_sent(n_old, s) := true
  table(n_old, k, v) := false
  owner(n_old, k) := false(*\label{kv-code:cede-own}*)
  transfer_msg(n_old, n_new, k, v, s) := true(*\label{kv-code:inserting-tuple}*)
  unacked(n_old, n_new, k, v, s) := true(*\label{kv-code:reshard-end}*)

action drop_transfer_msg(src:node, dst:node,(*\label{kv-code:transfer-drop-start}*)
                    k:key, v:value, s:seqnum)
    require transfer_msg(src, dst, k, v, s)(*\label{kv-code:requiring-tuple}*)
    transfer_msg(src, dst, k, v, s) := false(*\label{kv-code:removing-tuple}*)(*\label{kv-code:transfer-drop-end}*)

action retransmit(src:node, dst:node,(*\label{kv-code:transfer-retransmit-start}*)
                  k:key, v:value, s:seqnum)
    require unacked(src, dst, k, v, s)
    transfer_msg(src, dst, k, v, s) := true(*\label{kv-code:transfer-retransmit-end}*)
  \end{lstlisting}
  %\end{subfigure}%
  \end{minipage}
\hspace{0.0\textwidth}%
%\begin{subfigure}[t]{0.28\textwidth}
\begin{minipage}{0.4\textwidth}
  \begin{lstlisting}[numbers=left, numberstyle=\tiny, numbersep=5pt, name=lockserv, escapeinside={(*}{*)}]
action recv_transfer_msg(src:node, n:node,(*\label{kv-code:receive-transfer-start}*)
                         k:key, v:value, s:seqnum)
    require transfer_msg(src, n, k, v, s)
          $\land$$\neg$seqnum_recvd(n, src, s)(*\label{kv-code:ignore-dup}*)
    seqnum_recvd(n, src, s) := true
    table(n, k, v) := true
    owner(n, k) := true(*\label{kv-code:receive-transfer-end}*)

action send_ack(src:node, n:node,(*\label{kv-code:ack-start}*)
                k:key, v:value, s:seqnum)
    require transfer_msg(src, n, k, v, s)
          $\land$seqnum_recvd(n, src, s)
    ack_msg(src, n, s) := true(*\label{kv-code:ack-end}*)

action drop_ack_msg(src:node, dst:node,(*\label{kv-code:ack-drop-start}*)
                    k:key, s:seqnum)
    require ack_msg(src, dst, s)
    ack_msg(src, dst, s) := false(*\label{kv-code:ack-drop-end}*)

action recv_ack_msg(src:node, dst:node, 
                    k:key, s:seqnum)
    require ack_msg(src, dst, s)
    unacked(src, dst, *, *, s) := false(*\label{kv-code:qf-update:recv_ack_msg}*)

action put(n:node, k:key, v:value)
    require owner(n, k)
    table(n, k, *) := false(*\label{kv-code:qf-update:put}*)
    table(n, k, v) := true(*\label{kv-code:action-end}*)

safety $\forall k, n_1, n_2, v_1, v_2.$(*\label{kv-code:safety-start}*)
  table($n_1$,$k$,$v_1$) $\land$
  table($n_2$,$k$,$v_2$) $\to$
  $n_1 = n_2 \land v_1 = v_2$(*\label{kv-code:safety-end}*)
  \end{lstlisting}
%  \end{subfigure}
\end{minipage}
\captionof{figure}{\footnotesize Sharded key-value store with retransmissions (KV-R) in a first-order relational modeling.}
  \label{fig:kv-ivy}
  \end{minipage}
%  \begin{subfigure}[t]{0.3\textwidth}  %\caption{Lock service modeled in Ivy (left) and logical phase characterizations to prove it inductive (right) .}
\end{figure*} 

%\caption{Phase automaton for the lock service (left) and logical phase characterizations to prove it inductive (right).
%    Clockwise from top, the
%    phases for the lock $\lockelem$ are: Server Holds Lock, Grant message destined for some client, lock held by some client, and Unlock message sent from some client and pending to be received by the server.  The transitions are labeled by actions of the system. The wildcard \texttt{*} means that the action is executed by some arbitrary node.
%    %(in the transition relation this is translated to an existential quantifier).
%    Each phase has
%    a self loop for \texttt{send\_lock}, which can happen at any time. Actions related to locks other than $\lockelem$ are considered as self-loops, and omitted here for brevity. There
%    are four non-self-loop edges, forming the core of the automaton and
%    capturing the lifecycle of the lock service. Not all actions are allowed
%    in every phase: only those actions with outgoing edges are allowed. Our
%    inference algorithm exploits missing edges as additional safety properties
%    to guide the search.
%  }

==> figs/workflow.tex <==
\begin{figure}[t]
  \centering
  %\includegraphics[width=3in]{figs/lockserv-automaton-labeled-states}
  \includegraphics[width=\textwidth]{figs/workflow.jpg}
  \caption{The work-flow of user-guided invariant inference through phase structures.
  The input to the tool is a (1) program, (2) safety property, and (3) phase structure.
  The output is either (4) inductive phase characterizations over the given phase structure, or (5) proof that universally quantified inductive phase characterizations do not exist, in the form of an abstract trace.
  }
  \label{fig:workflow}
\end{figure}

